Spatio-Spectral Graph Neural Networks

Spatial Message Passing Graph Neural Networks (MPGNNs) are widely used for learning on graph-structured data. However, key limitations of l-step MPGNNs are that their "receptive field" is typically limited to the l-hop neighborhood of a node and that information exchange between distant nodes is limited by over-squashing. Motivated by these limitations, we propose Spatio-Spectral Graph Neural Networks (S$^2$GNNs) -- a new modeling paradigm for Graph Neural Networks (GNNs) that synergistically combines spatially and spectrally parametrized graph filters. Parameterizing filters partially in the frequency domain enables global yet efficient information propagation. We show that S$^2$GNNs vanquish over-squashing and yield strictly tighter approximation-theoretic error bounds than MPGNNs. Further, rethinking graph convolutions at a fundamental level unlocks new design spaces. For example, S$^2$GNNs allow for free positional encodings that make them strictly more expressive than the 1-Weisfeiler-Lehman (WL) test. Moreover, to obtain general-purpose S$^2$GNNs, we propose spectrally parametrized filters for directed graphs. S$^2$GNNs outperform spatial MPGNNs, graph transformers, and graph rewirings, e.g., on the peptide long-range benchmark tasks, and are competitive with state-of-the-art sequence modeling. On a 40 GB GPU, S$^2$GNNs scale to millions of nodes.

==> tabulars/source_dist.tex <==
\begin{tabular}{lccrr}
\toprule
 & \begin{tabular}{@{}c@{}}+ Spec.\\ filter\end{tabular} & \(\PE\) & \textbf{ID} $R^2 \, (\uparrow)$ & \textbf{OOD} $R^2 \, (\uparrow)$ \\
\midrule
\multirow[c]{6}{*}{\rotatebox{90}{\textbf{DAGs}}} & \xmark & \xmark & $0.1915 \pm 0.0001$ & $0.1214 \pm 0.0066$ \\
 & \xmark & \cmark & $0.2322 \pm 0.0004$ & $0.1745 \pm 0.0003$ \\
  & undir. & \xmark & $0.8956 \pm 0.0006$ & $0.8148 \pm 0.0020$ \\
 & undir. & \cmark & $0.9124 \pm 0.0003$ & $0.8410 \pm 0.0008$ \\
 & direc. & \xmark & \underline{$0.9544 \pm 0.0014$} & \underline{$0.8924 \pm 0.0040$} \\
 & direc. & \cmark & $\mathbf{0.9592 \boldsymbol{\pm} 0.0003}$ & $\mathbf{0.9025 \boldsymbol{\pm} 0.0024}$ \\
\midrule
\multirow[c]{6}{*}{\rotatebox{90}{\textbf{Trees}}} & \xmark & \xmark & $0.0958 \pm 0.0029$ & $0.0144 \pm 0.0127$ \\
 & \xmark & \cmark & $0.3262 \pm 0.0022$ & $0.2110 \pm 0.0050$ \\
  & undir. & \xmark & $0.9902 \pm 0.0020$ & $0.9839 \pm 0.0053$ \\
 & undir. & \cmark & $0.9878 \pm 0.0031$ & $0.9856 \pm 0.0055$ \\
 & direc. & \xmark & \underline{$0.9944 \pm 0.0060$} & \underline{$0.9881 \pm 0.0069$} \\
 & direc. & \cmark & $\mathbf{0.9954 \boldsymbol{\pm} 0.0041}$ & $\mathbf{0.9938 \boldsymbol{\pm} 0.0077}$ \\
\bottomrule
\end{tabular}

==> trash.tex <==



Old Intro


\iffalse
\textbf{\nameacr{} generalize ``virtual nodes'' and vanquish over-squashing.}  A so-called virtual node~\citep{gilmer_neural_2017,battaglia_relational_2018,cai_connection_2023} is connected to all regular nodes of the graph to allow for a global exchange of messages, \nameacr{} contain this as a special case while modeling more sophisticated global interactions. Moreover, we prove and empirically verify in \autoref{sec:oversquashing} that combining spectral and spatial filters alleviates the over-squashing phenomenon~\citep{alon_bottleneck_2020,di2023over, di_giovanni_how_2023}. %


\textbf{SpecSpat is \todo{optimal} for approximating the true filter.} \todo{We show how \(p_{\text{cut}}\) and \(\eigval_{\text{cut}}\) should be scaled to each other such that the approximation error has a constant upper bound, assuming that the true filter is integral Lipschitz. Integral Lipschitzness is a necessary property to obtain stable graph filters in the sense of~\citet{gama_stability_2020}.}

\textbf{\nameacr{} unlock new design spaces.}

\textbf{(C)}
\textbf{SpecSpat is strictly more expressive than 1-WL.} We propose the first efficient spectral positional encoding (linear in the number of edges \(m\)) that yields a strictly greater expressivity than the 1-WL (\autoref{sec:pos_enc}). It is simple and has negligible computational cost in combination with SpecSpat.

\textbf{(D)}
\textbf{SpecSpat unlocks new design spaces.} Revisiting spectral graph convolutions unlocks unexplored design spaces for GNNs. For example, we propose a permutation-equivariance-preserving neural network for the spectral domain with interesting scaling properties~\autoref{sec:nn_spec}, and we propose the first spectral filter for directed graphs in~\autoref{sec:directed_spectral_filter}.

\textbf{(E)}
\textbf{SpecSpat is effective and efficient.} We show in carefully designed experiments the shortcomings of MPGNNs and how SpecSpat overcomes them (\autoref{sec:results}). For example, we set a new state-of-the-art on the peptides-func benchmark~\citep{dwivedi_long_2023} with \(\approx\)\,40\% fewer parameters. Thus, SpecSpat outperforms state-of-the-art MPGNNs (potentially applied to a rewired graph), as well as graph transformers. Our spectral filter requires a partial eigendecomposition and scales linearly in the number of nodes \(n\) and the number of eigenvectors \(k\). The partial eigendecomposition is in \(\mathcal{O}(k m)\) with the number of edges \(m\) and is required once per graph. Thus, SpecSpat can have an identical computational complexity to purely spatial MPGNN. Vanilla full-graph training of SpecSpat allows for learning on millions of nodes with a 40\,GB GPU.




\iffalse
So far, we have treated the polynomial order $p$ and cutoff eigenvalue $\lambda_\text{max}$ as constants independent of the input graph.The number of eigenvalues in $[0, \lambda_\text{max}]$ then grows linearly with the node count $n$, leading to an overall quadratic scaling which may be impractical for large-scale graphs. However, a key strength of \namefull{} is that $\lambda_\text{max}$ and the polynomial order $p$ can be flexibly adapted to the problem scale (decreasing $\lambda_\text{max}$ with $n$, while possibly increasing $p$ to compensate), allowing for a flexible balance between accuracy and scaling. If the goal is having at most constant error, the following result holds (we formalize ``limiting eigenvalue densities'' in terms of graphons in \todo{link}):
\begin{theorem}[informal]
    \label{thm:scalinganalysis}
    For all possible graph sequences with the same limiting density of eigenvalues $\rho\colon [0,2] \to \sR$ and bound $K_r(\hat g, \lambda_\text{cut})$ as in \cref{thm:approximationtheory_basic}, scaling rules $n \mapsto \lambda_\text{max}\left(n; \hat g, \rho\right)$ and $n \mapsto p\left(n; \hat g, \rho\right)$ the approximation error remains bounded by a constant,
    \[\sup_{0 \neq \bm X \in \sR^{n \times d}}\frac{\lVert(g_{\bm{\gamma}_{p\left(n; \hat g \rho\right)}^*} + g_{\vartheta^*;n}-g) \ast_{\gG_n} \bm{X}\rVert_2}{\lVert \bm{X} \rVert_2} = \mathcal{O}\left(1\right),\]
    while the compute cost is of $\mathcal{O}\left(n^{\beta(\hat g, \rho)}\right)$ with $1 \leq \beta(\hat g, \rho) \leq 2$.

    
\end{theorem}
We remark that the worst-case quadratic scaling, not excluded by \cref{thm:scalinganalysis}, occurs only the pathological edge case in which all nodes in  $(\mathcal{G}_n)_{n \in \sN}$ are disconnected such that $\rho$ is a Dirac delta at 0 and reducing $\lambda_{\max}$ brings no cost benefit at all. Otherwise, the method is strictly subquadratic at constant error, thereby surpassing fully connected long-range approaches in efficiency while also satisfying theoretical guarantees.

\textbf{Setup.} We compare the expressiveness of \nameacr{} against a more powerful class of ``idealized'' GNNs (\textit{IGNNs}) containing $L$ graph convolution layers $1 \leq l \leq L$, each of which can express \textit{any} filter bank $g\layer \in \sR^{n \times d\Layer}$, represented spectrally as a stack of $d\Layer$ arbitrary functions $\hat g\layer \colon \, [0,2] \to \sR^{d\Layer}$. An IGNN layer in our framework therefore has the generic structure
\begin{equation*}
    \mH\Layer = \sigma\left(g\layer \ast_\gG [\mH\layer \mW\layer]\right) = \sigma\left(\mV \hat g\layer(\veigval) \odot [\mV^\top \mH\layer \mW\layer]\right).
\end{equation*}
Given this theoretical baseline which can express arbitrary filters, we study how quickly the predictions of the closest-approximating \nameacrsing{} with $\ell$ spatio-spectrally parametrized filter convolutions converge to the IGNN predictions (uniformly across graphs and input signals) as we take $\ell \rightarrow \infty$. We assume the additive form from \autoref{eq:specspat} with $\ell \geq L$ layers, a spectral filter as in \autoref{eq:spec} which is fully supported on a low-pass window of eigenvalues $[0, \lambda_\text{cut}]$ but satisfies universal approximation in this window, and a spatial part of the form
\[\spat^{(l)}(\mH^{(l-1)}; \mA) = \sigma\left(\left[\sum_{j=0}^{p\Layer}\mL^j\bm{\gamma}_j^\top\right] \mH^{(l-1)} \mW\layer \right)\]
with polynomial orders $p\Layer$ and learnable coefficient vectors $\bm{\gamma} = [\bm{\gamma}_1, \dots, \bm{\gamma}_{p\Layer}] \in \sR^{d \times {p\Layer}}$. The outer product with $\bm{\gamma}_j^\top$ compactly denotes that each hidden dimension $1 \leq i \leq d$ of $\sum_{j=0}^{p\Layer} \mL^j\bm{\gamma}_j^\top \in \sR^{n \times n \times d}$ gets its own polynomial with coefficients $(\gamma_j)_i$. Architectures such as ChebNet \citep{defferrard_convolutional_2017}, BernNet \citep{he_bernnet_2021}, or GCN \citep{kipf_semi-supervised_2017} arise as a special case by tying coefficients across hidden dimensions, and then either reparametrizing in terms of a different polynomial basis or entirely fixing coefficients.\par
\textbf{Linear simplification}. From a modeling standpoint, we can think of the fixed $L$-layer IGNN as an expressive proxy for an unknown ground truth. It captures a wide host of (potentially long-ranged) interactions: in fact, \citet{wang_how_2022} prove that even linear IGNNs can produce any one-dimensional output under certain regularity assumptions on the graph and input signal. For both notational and conceptual simplicity, we focus the main body on this linear case, i.e., set $\sigma = \mI$, such that $L$ IGNN layers collapse to a single filter $g$. Likewise, an $\ell$-layer \nameacrsing{} collapses to a simple convolution layer with two additive parts,
\[\mH^{(\ell)} = (g_{{\bm{\gamma}}} + g_\vartheta) \ast_\gG \mH^{(0)} = \left[\sum_{j=0}^{p} \mL^j \bm{\gamma}_j^\top\right] \mH^{(0)} \mW_{\spat} + \mV \hat g_\vartheta(\veigval) \odot [\mV^\top \mH^{(0)} \mW_{\spec}]\]
with total polynomial order $p = \sum_{l=1}^\ell p\Layer$. In essence, we want to assess the approximation-theoretic benefits of adding a low-pass-supported, but otherwise arbitrarily expressive filter $g_\vartheta$ to a standard polynomial filter $\sum_{j=0}^{p} \mL^j \bm{\gamma}_j^\top$ with full frequency support but limited spectral selectivity due to its finite polynomial degree $p$, based on the smoothness structure of the ``ideal'' filter $g$.\todo{Link to full treatment including nonlinearities in appendix}\par
\textbf{Spectral smoothness guarantees accuracy.} Intuitively, the range of the ideal filter $g$ is related to the smoothness of its Fourier transform $\hat g$. For instance, if $g$ is a low-order polynomial of $\mL$, it is localized to a few-hop neighborhood, and $\hat g$ is regularized to vary slowly in its argument. The other extreme is a discontinuous spectral filter $ \hat g$, such as the entirely non-local virtual node filter (details in \autoref{app:virtualnode}), $\hat g = \mathds{1}_{\{0\}}$, with $\mathds{1}_{\mathcal{S}}$ denoting the indicator function of a set $\mathcal{S}$. This viewpoint of spectral smoothness illuminates the limitations of finite-hop message passing from an angle alternative to prior spatial analyses in the over-squashing framework. It admits a lower error bound, which shows that polynomial-filter graph convolutions converge exceedingly slowly to a spectrally-discontinuous ground truth in terms of their induced operator norm:
\begin{theorem}
\label{thm:discontinuous}
    Given a discontinuous filter bank $\hat g \colon [0,2] \to \sR^d$ and an approximating sequence $\left(\hat g_{\bm{\gamma}_p} \colon [0,2] \to \sR^d, \, \lambda \mapsto \sum_{j=0}^{p} \bm{\gamma}_j \lambda^j\right)_{p \in \sN}$ with arbitrary coefficients $\bm{\gamma}_p = [\bm{\gamma}_1, \dots, \bm{\gamma}_{p}] \in \sR^{d \times p}$,\newline
    an adversarial graph sequence $(\mathcal{G}_p)_{p \in \sN}$ exists such that 
    \[\nexists \alpha \in \sR^+ \colon \, \sup_{0 \neq \bm X \in \sR^{|\mathcal{G}_p| \times d}}\frac{\lVert(g_{\bm{\gamma}_p}-g) \ast_{\gG_p} \bm{X}\rVert_2}{\lVert \bm{X} \rVert_2} = \mathcal{O}\left(p^{-\alpha}\right).\]
\end{theorem}
Revisiting the example of the discontinuous virtual node filter, we spot a sharp contrast to the properties of \nameacr{} which yield perfect accuracy even with an arbitrarily small $\lambda_\text{max}$. More generally, a spatio-spectral convolution wins over its purely spatial counterpart when the sharpest irregularities of the ground truth $\hat g$ happen to be caught within its window of perfect reconstruction. The spatial part, which can ``focus'' on learning the remaining, smoother part outside of this window, now needs much fewer hops to yield a faithful approximation. Formally, we find:
\begin{theorem}
\label{thm:approximationtheory_basic}
    Given a low-pass window $[0, \lambda_{\text{cut}}]$ with $\lambda_{\text{cut}} \in (0,2)$, a filter bank $\hat g \colon [0,2] \to \sR^d$ and its restriction $\hat g = \hat g \big \lvert_{[\lambda_{\text{cut}}, 2]}$, assume that a continuous $r$-th derivative $\dr \hat g$ of $\hat g$ and a bound $K_r(\hat g, \lambda_\text{cut}) \in \sR^+$ exist such that $\left \lvert \dr \hat g_i(\lambda) \right \rvert \leq K_r(\hat g, \lambda_\text{cut}) \, \, \forall \lambda \in [\lambda_{\text{cut}}, 2]$, $1 \leq i \leq d$.\par
    A spectral part $g_{\vartheta^*}$ and an approximating sequence $\left(\hat g_{\bm{\gamma}_p^*} \colon [0,2] \to \sR^d, \, \lambda \mapsto \sum_{j=0}^{p} \bm{\gamma}_j^* \lambda^j\right)_{p \in \sN}$ with coefficients $\bm{\gamma}^*_p = [\bm{\gamma}_1^*, \dots, \bm{\gamma}_{p}^*] \in \sR^{d \times p}$ exist such that, for all graph sequences $(\mathcal{G}_p)_{p \in \sN}$,
    \[\sup_{0 \neq \bm X \in \sR^{|\mathcal{G}_p| \times d}}\frac{\lVert(g_{\bm{\gamma}_p^*} + g_{\vartheta^*}-g) \ast_{\gG_p} \bm{X}\rVert_2}{\lVert \bm{X} \rVert_2} \leq C_r K_r(\hat g, \lambda_\text{cut}) p^{-r} = \mathcal{O}\left(p^{-r}\right),\]
    with a constant $C_r > 0$ that depends only $r$, not on $\hat g$ or $(\mathcal{G}_p)_{p \in \sN}$.
\end{theorem}
\begin{wrapfigure}[17]{r}{0.5\textwidth}
    \vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{resources/spec_spat_contrast_capabilities.pdf}
    \caption{We show the additive combination (right) of examples of \todo{adversarial filters} for spectral (left) and spatial (middle) filters. Moreover, a \nameacrsing{} is able to perfectly approximate the true filter in all cases.}
    \label{fig:spec_spat_contrast}
\end{wrapfigure}
We note that the above bound extends to purely spatial convolutions in terms of $K_r(\hat g, 0)$ if $\hat g$ is $r$-times continuously differentiable on the full interval $[0,2]$. The \nameacrsing{} bound of \autoref{thm:approximationtheory_basic} is still strictly tighter if $K_r(\hat g, \lambda_\text{cut}) < K_r(\hat g, 0)$. In particular, taking the limit $K_1(\hat g, 0) \to \infty$ towards discontinuity makes the purely spatial upper bound arbitrarily loose, whereas a benign filter might still admit a small $K_1(\hat g, \lambda_\text{cut})$ for some $\lambda_\text{cut} > 0$. The lower bound of \autoref{thm:discontinuous} demonstrates that this is not simply an artifact of a loose upper bound, but that there is an inherent difficulty in approximating discontinuous filters with polynomials.\par
\textbf{The case for low-pass windows.} An obvious remaining question is why the window of perfect reconstruction should be in a low-pass band $[0, \lambda_\text{max}]$ rather than, say, a high-pass band $[\lambda_\text{min}, 2]$. Indeed, if domain-informed considerations suggest that this is where the ground-truth interactions have the highest spectral selectivity, our method should be adapted accordingly (analogous approximation-theoretic results also hold in this case). However, such knowledge is rarely available. As an exception to this rule, we do construct an explicit filter $\hat g_\sigma$ modeling electrostatic interactions in a periodic chain of screened charges in \todo{link}, and find that a low-pass window is indeed optimal. A reasonable prior in the absence of such evidence stems from the observation that graphs are often discrete samples of an underlying continuous phenomenon \citep{levie_transferability_2021}, and hence predictions should be robust to small perturbations of the graph structure. \citet{gama_stability_2020} find that, under a relative perturbation model (allocating perturbation budget in proportion to connectivity), stability implies integral Lipschitzness:
\[\exists C(\hat g) \geq 0\colon \, |\hat g_i(\lambda_2) - \hat g_i(\lambda_1)| \leq C(\hat g)\frac{|\lambda_2 - \lambda_1|}{|\lambda_1+\lambda_2|/2} \, \forall \lambda_1 \neq \lambda_2 \in [0,2], \, 1 \leq i \leq d.\]
For differentiable filters, this implies $|\lambda \hat g^{(1)}_i(\lambda)| \leq C(\hat g)$: the filter can vary arbitrarily rapidly around zero but must level out towards larger $\lambda$. Unlike for standard Lipschitzness (the appropriate regularization criterion under an absolute perturbation model), imposing relative stability and thus integral-Lipschitz filters allows for stable yet expressive IGNN baselines: As \citep{gama_stability_2020} argue, nonlinearities can ``spill'' features into lower frequency ranges where an integral-Lipschitz IGNN (as well as the spectral part of an approximating \nameacrsing{}) is arbitrarily selective. In terms of \autoref{thm:approximationtheory_basic}, imposing integral Lipschitzness yields a bound with $r=1$ and $K_1(\hat g, \lambda_\text{cut}) = \frac{C(\hat g)}{\lambda_\text{cut}}$. While this generic prior constrains only the first derivative, concrete applications might inform additional smoothness criteria, leading to sharper bounds on the convergence rate. In the electrostatics example of \todo{link}, we find\footnote{The bound is not tight enough for $r=1$ and small $\lambda$ to also certify integral Lipschitzness for this example. It holds nonetheless, as we verify separately in \todo{link}.} $K_r(\hat g_\sigma, \lambda) \propto \frac{r!}{\lambda^{(r+1)}}$.\todo{Evtl.: Generalizing self-attention as another reason for low-frequency window.}\par
\textbf{Scaling analysis.} So far, we have treated the polynomial order $p$ and cutoff eigenvalue $\lambda_\text{max}$ as constants independent of the input graph. The number of eigenvalues in $[0, \lambda_\text{max}]$ then grows linearly with the node count $n$, leading to an overall quadratic scaling which may be impractical for large-scale graphs. However, a key strength of \namefull{} is that $\lambda_\text{max}$ and the polynomial order $p$ can be flexibly adapted to the problem scale (decreasing $\lambda_\text{max}$ with $n$, while possibly increasing $p$ to compensate), allowing for a flexible balance between accuracy and scaling. If the goal is having at most constant error, the following result holds (we formalize ``limiting eigenvalue densities'' in terms of graphons in \todo{link}):
\begin{theorem}[informal]
    \label{thm:scalinganalysis}
    Let $\mathcal{S}[\rho]$ denote the set of all graph sequences $(\mathcal{G}_n)_{n \in \sN} \in \mathcal{S}[\rho]$ with $|\mathcal{G}_n| = n$ converging to the same limiting density of eigenvalues $\rho\colon [0,2] \to \sR$. Assume a bound $K_r(\hat g, \lambda_\text{cut})$ as in \cref{thm:approximationtheory_basic}. Scaling rules $n \mapsto \lambda_\text{max}\left(n; \hat g, \rho\right)$ and $n \mapsto p\left(n; \hat g, \rho\right)$, and according spatio-spectral convolutions with spectral part $g_{\vartheta^*;n}$ and spatial parts $\left(\hat g_{\bm{\gamma}_{p\left(n; \hat g, \rho\right)}^*}\right)_{n \in \sN}$ exist such that, for all $(\mathcal{G}_n)_{n \in \sN} \in \mathcal{S}[\rho]$, the approximation error remains bounded by a constant,
    \[\sup_{0 \neq \bm X \in \sR^{n \times d}}\frac{\lVert(g_{\bm{\gamma}_{p\left(n; \hat g \rho\right)}^*} + g_{\vartheta^*;n}-g) \ast_{\gG_n} \bm{X}\rVert_2}{\lVert \bm{X} \rVert_2} = \mathcal{O}\left(1\right),\]
    while the compute cost is of $\mathcal{O}\left(n^{\beta(\hat g, \rho)}\right)$ with $1 \leq \beta(\hat g, \rho) \leq 2$.
\end{theorem}
We remark that the worst-case quadratic scaling, not excluded by \cref{thm:scalinganalysis}, occurs only the pathological edge case in which all nodes in  $(\mathcal{G}_n)_{n \in \sN}$ are disconnected such that $\rho$ is a Dirac delta at 0 and reducing $\lambda_{\max}$ brings no cost benefit at all. Else, the method is strictly subquadratic at constant error, thereby surpassing fully-connected long-range approaches in efficiency while also satisfying theoretical guarantees.



\fi



\begin{wraptable}[10]{r}{0.1675\textwidth}
    \RawFloats
    \vspace{-15pt}
    \caption{Kendall tau rank correlation on joint TPUGraphs ``layout'' (val.).}
    \label{tab:tpu_graphs}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lr}
    \toprule
    GCN & $60.09$ \\
    \nameprefix GCN & $65.74$ \\
    \bottomrule
    \end{tabular}}
\end{wraptable}

\begin{wraptable}[10]{r}{0.4\textwidth}
    \RawFloats
    \vspace{-15pt}
    \caption{OGB Products.}
    \label{tab:results_products}
    \centering
    \resizebox{\linewidth}{!}{
        \input{tabulars/products}
    }
\end{wraptable}

\begin{wraptable}[10]{r}{0.4\textwidth}
    \RawFloats
    \vspace{-15pt}
    \caption{30k token associative recall.}
    \label{tab:results_assoc_recall_large}
    \centering
    \resizebox{\linewidth}{!}{
        \input{tabulars/associative_recall_30k}
    }
\end{wraptable}

\begin{wrapfigure}[18]{r}{0.25\textwidth}
    \vspace{-15pt}
    \centering
    \includegraphics[width=\linewidth]{resources/associative_recall_small.pdf}\\
    \caption{\nameprefix GCN solves associative recall for sequences varying in size by two orders of magnitude. The grey area marks \textbf{ID}.}
    \label{fig:results_assoc_recall_small}
\end{wrapfigure}

\begin{wrapfigure}[13]{r}{0.43\textwidth}
    \centering
    \vspace{-12pt}
    \includegraphics[width=0.58\linewidth]{resources/runtime_legend.pdf}\\
    \vspace{-16pt}
    \subfloat[\texttt{scipy}]{\includegraphics[width=0.47\linewidth]{resources/runtime_cpu.pdf}\label{fig:runtime_scipy}}
    \vspace{5pt}
    \subfloat[\texttt{PyTorch}]{\includegraphics[width=0.49\linewidth]{resources/runtime_gpu.pdf}\label{fig:runtime_pytorch}}
    \vspace{-10pt}
    \caption{Runtime of partial eigendecomposition \(k=25\) of Erd\H{o}s R\'enyi graph with average degree 5. Dashed mark directed/Hermitian Laplacian.\label{fig:runtime}}
\end{wrapfigure}

\begin{wrapfigure}[18]{r}{0.3\textwidth}
    \vspace{-15pt}
    \centering
    \includegraphics[width=\linewidth]{resources/di_givanni_extended.pdf}\\
    \caption{Extension of the over-squashing experiment of \citet{di2023over} to larger graphs and an equal mix of ``Ring'' and ``CliquePath'' graphs. We compare a 15-layer (largest number of layers that trains stably) GatedGCN~\citep{bresson_residual_2018} (\(\spat\)) with a single spectral filter (\(\spec\)). The grey shaded area marks the training distribution.}
    \label{fig:di_givanni_extended}
\end{wrapfigure}


\begin{wrapfigure}[15]{r}{0.6\textwidth}
    \RawFloats
    \centering
    \vspace{-27pt}
    \begin{minipage}{0.62\textwidth}
        \captionsetup{type=table}
        \captionsetup{margin=0.3cm}
        \caption{$R^2$ on the distance task, with DirGCN as MPGNN. The best mean score is bold, second is underlined. \label{tab:source_dist_results}}
        \centering
        \resizebox{\linewidth}{!}{
            \input{tabulars/source_dist}
        }
    \end{minipage}%
    \hfill
    \begin{minipage}{0.36\textwidth}
        \captionsetup{margin=0.3cm}
        \centering
        \includegraphics[width=\linewidth]{resources/source_dist_dagext_rmse_preds.pdf}
        \vspace{-15pt}
        \caption{RMSE and 90\% pred. intervals of distances by ground truth on OOD DAGs.}
        \label{fig:source_dist_rmse_preds}
    \end{minipage}
    \vspace{-18pt}
\end{wrapfigure}

\begin{figure}
    \RawFloats
    \centering
    \begin{minipage}{0.43\textwidth}
        \vspace{-5pt}
        \captionsetup{type=table}
        \caption{Results on the \texttt{CLUSTER} task~\citep{dwivedi_benchmarking_2022}. Transformer models that outperform our \nameprefix GatedGCN are underlined. \label{tab:cluster_sbm}}
        
        \centering
        \resizebox{\linewidth}{!}{
            \input{tabulars/cluster_sbm}
        }
    \end{minipage}%
    \hfill
    \begin{minipage}{0.55\textwidth}
        \captionsetup{type=figure}
        \centering
        \vspace{-12pt}
        \subfloat[Vary \# of eigenvectors \(k\) for 4 spatial MP layers.]{\includegraphics[width=0.47\linewidth]{resources/cluster_gmm_num_eigvecs.pdf}\label{fig:cluster_gmm_num_eigvecs}}
        \vspace{5pt}
        \subfloat[Vary \# of spatial MP layers \textcolor{plt-C1}{w/} or \textcolor{plt-C0}{w/o} one spectral layer.]{\includegraphics[width=0.49\linewidth]{resources/cluster_gmm_layers.pdf}\label{fig:cluster_gmm_layers}}
        \vspace{-10pt}
        \caption{Performance of \nameprefix GCN on the GMM clustering task. Solid lines are w/, dashed lines are w/o our $\PE$ (\autoref{sec:pos_enc}).}
    \end{minipage}
    \vspace{-18pt}
\end{figure}

\begin{wrapfigure}[14]{r}{0.6\textwidth}
    \vspace{-15pt}
    \centering
    \sidesubfloat[]{\includegraphics[width=0.93\linewidth]{resources/cluster_sbm_filters.pdf}}
    \hfill
    \sidesubfloat[]{\includegraphics[width=0.93\linewidth]{resources/cluster_gmm_filters.pdf}}
    \caption{SBM-based (a) and \emph{our} GMM-based (b) graphs along with four learned filters. Large entries are yellow, small are blue, and white lines denote clusters.}
    \label{fig:cluster_filters}
\end{wrapfigure}


\begin{wrapfigure}[11]{r}{0.6\textwidth}
    \centering
    \vspace{-25pt}
    \subfloat[]{\includegraphics[width=0.3\linewidth]{resources/cluster_gmm_graph_0.pdf}}
    \subfloat[]{\includegraphics[width=0.3\linewidth]{resources/cluster_gmm_graph_1.pdf}}
    \subfloat[]{\includegraphics[width=0.3\linewidth]{resources/cluster_gmm_graph_2.pdf}}
    \caption{Examples of generated graphs for the GMM clustering task. Labeled nodes are marked \textcolor{red}{red}.\label{fig:cluster_gmm_example_graphs}}
\end{wrapfigure}

\begin{wrapfigure}[12]{r}{0.6\textwidth}
    \vspace{-25pt}
    \centering
    \subfloat[]{\includegraphics[width=0.3\linewidth]{resources/cluster_sbm_graph_0.pdf}}
    \subfloat[]{\includegraphics[width=0.3\linewidth]{resources/cluster_sbm_graph_1.pdf}}
    \subfloat[]{\includegraphics[width=0.3\linewidth]{resources/cluster_sbm_graph_2.pdf}}
    \caption{Examples of generated graphs for the SBM clustering task. Labeled nodes are marked \textcolor{red}{red}. Edges within clusters are highlighted.\label{fig:cluster_sbm_example_graphs}}
\end{wrapfigure}



\subsection{Global Residual Readouts}\label{app:global_residual}


The architecture for graph-level tasks is sketched in \autoref{fig:architecture}. The node embeddings \(\mH^{(l)} \in \R^{n \times d}\) are successively processed by spatial and spectral filters. 

\textbf{Spectral readout.} Each spectral layer allows for a rich yet computationally cheap readout of graph-level information. For this, we take the absolute value of \(|\mY|\) defined in \autoref{eq:spec}. This way, each spectral layer contributes to the final graph embedding. All the global embeddings are collected and then stacked for the final prediction using an MLP.

\begin{figure}[b]
    \centering
    \includegraphics[width=0.75\linewidth]{resources/architecture_2.pdf}
    \caption{3-layer \nameacrsing{} architecture overview for graph-level tasks}
    \label{fig:architecture}
\end{figure}

\textbf{Input encoding.} Before the graph convolutions, we use a 2-layer MLP to embed the node features. The Encoder is similar to the sample code but adds the different inputs projected to \(d\) dimensions instead of concatenating them. The edge features \(\mE\) are encoded using a linear layer on top of sinusoidal encodings for the edge order.

\textbf{Computational cost.} Despite the flexibility, the architecture is relatively light-weight and trains on a single 40GB A100. Specifically, on the layout XLA random task, we set the inner dimensions to \(d=96\), and each batch contains a single graph but at least 56 configurations (see \autoref{sec:results} for more details). We scale the number of batched configurations inversely to the number of nodes \(n\) to improve the GPU utilization on smaller graphs.

\begin{wrapfigure}[15]{r}{0.42\textwidth}
    \vspace{-16pt}
    \centering
    \includegraphics[width=\linewidth]{resources/spec_spat_contrast_capabilities.pdf}\\\vspace{-8pt}
    \caption{We show the additive combination (right) of examples of difficult to model filters for spectral (left) and spatial (middle) filters. Moreover, a \nameacrsing{} is able to perfectly approximate the true filter in all cases.}
    \label{fig:spec_spat_contrast}
\end{wrapfigure}



